VLRM: Vision-Language Models act as Reward Models for Image Captioning

In this work, we present an unsupervised method for enhancing an image captioning model (in our case, BLIP2) using reinforcement learning and vision-language models like CLIP and BLIP2-ITM as reward models. The RL-tuned model is able to generate longer and more comprehensive descriptions. Our model reaches impressive 0.90 R@1 CLIP Recall score on MS-COCO Carpathy Test Split. Weights are available at https://huggingface.co/sashakunitsyn/vlrm-blip2-opt-2.7b.

==> imgs/plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Training steps},
xmin=-117.5, xmax=2467.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={COCO R@1},
ymin=25, ymax=95,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 38.819998
50 46.859998
100 55.233331
150 52.619996
200 47.553333
250 34.9
300 28.44
350 47.233334
400 52.199999
450 59.359998
500 62.019999
550 61.199997
600 63.213333
650 70.073331
700 71.886665
750 76.09333
800 75.706665
850 72.973328
900 73.266663
950 75.539998
1000 70.126666
1050 77.913335
1100 78.359998
1150 77.633334
1200 78.426664
1250 78.899996
1300 79.779994
1350 78.133334
1400 76.659999
1450 79.173327
1500 79.746663
1550 80.106664
1600 78.446665
1650 80.426664
1700 79.366661
1750 80.513331
1800 80.426664
1850 81.579997
1900 81.506663
1950 80.753332
2000 81.786664
2050 82.906665
2100 82.82
2150 81.679998
2200 83.046666
2250 81.806664
2300 76.659999
2350 75.293332
};
\addlegendentry{Single FC}
\addplot [semithick, darkorange25512714]
table {%
0 38.533334
50 55.013331
100 59.639998
150 60.82
200 63.853333
250 65.753334
300 64.699999
350 66.699994
400 68.326663
450 71.713336
500 70.526667
550 71.713333
600 72.719996
650 75.239998
700 76.646665
750 75.426664
800 78.073334
850 78.866664
900 79.953328
950 78.899999
1000 78.859998
1050 79.926664
1100 79.926664
1150 81.29333
1200 81.779996
1250 82.466665
1300 81.993332
1350 80.639994
1400 81.453331
1450 81.433332
1500 81.839999
1550 82.959999
1600 73.806664
1650 84.653333
1700 84.579999
1750 85.526662
1800 85.126661
1850 85.319995
1900 85.499992
1950 85.179995
2000 85.039996
2050 84.97333
2100 85.053329
2150 84.413333
2200 85.459997
2250 85.313327
2300 85.933329
2350 85.979996
};
\addlegendentry{Ours}
\end{axis}

\end{tikzpicture}

